Use Perturbations when Learning from Explanations

Machine learning from explanations (MLX) is an approach to learning that uses human-provided explanations of relevant or irrelevant features for each input to ensure that model predictions are right for the right reasons. Existing MLX approaches rely on local model interpretation methods and require strong model smoothing to align model and human explanations, leading to sub-optimal performance. We recast MLX as a robustness problem, where human explanations specify a lower dimensional manifold from which perturbations can be drawn, and show both theoretically and empirically how this approach alleviates the need for strong model smoothing. We consider various approaches to achieving robustness, leading to improved performance over prior MLX methods. Finally, we show how to combine robustness with an earlier MLX method, yielding state-of-the-art results on both synthetic and real-world benchmarks.

==> th_results.tex <==
\section{Theoretical Motivation}
\label{sec:th}

Introduce LMS-3 and LMS data, specifications.
Explain why it is a good dataset to study

\begin{figure*}[htb]
\begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{plots/LMS_plots/data.png}
    \caption{LMS data}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{plots/LMS_plots/LMS_reg=1_0.png}
    \caption{\rrr{}, $\lambda=0$}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{plots/LMS_plots/LMS_reg=1_0.1.png}
    \caption{\rrr{}, $\lambda=0.1$}
\end{subfigure}\hfill
\begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{plots/LMS_plots/LMS_reg=2_0.png}
    \caption{Perturbation, $\lambda=0$}
\end{subfigure}
\caption{(a) First two coordinates of LMS data. We wish to learn a classifier that is free of the linear feature shown on x-axis. Remaining plots show decision boundaries when fitted using different algorithms. (b) ERM only exploits linearly classifiable x-coordinate although it is possible to perfectly classify using the y-coordinate. (c) Despite explicit regularization, the fitted model still only exploits the x-coordinate. (d) Perturbations learn the desired classifier with the same supervision. \JH{This figures look so good! Why do decision boundaries(black) have dots instead of lines?}} 
\label{fig:toy}
\end{figure*}

\begin{theorem}[\cite{shah2020pitfalls}]
\label{th:lms_result}
Let $f(x) = \sum_{j=1}^k v_jReLU(\sum_{p=1}^d w_{p,j}x_p)$ denote a one-hidden-layer neural network with k hidden units and ReLU activations. Set $v_j = \pm 1/\sqrt{k}$ w.p. 1/2 $\forall j \in [k]$. Let $\{(x_i,y_i)\}_{i=1}^m$
denote i.i.d. samples from LSN where m $\in [cd^2, d^\alpha/c]$ for some $\alpha>2$. Then, given $d > \Omega(k\log k)$ and initial $w_{ij} \sim \mathcal{N}(0, 1)$, after O(1) iterations, mini-batch gradient descent (over w) with hinge loss, step size 
$\eta = \Omega(\log d)^{-1/2}$, mini-batch size
$\Theta(m)$. The learned weights of hidden units $w_{ij}$ satisfy:
\begin{align*}
    |w_{1j}| = \frac{2}{\sqrt{k}}(1-\frac{c}{\sqrt{\log d}}) + O(\frac{1}{\sqrt{dk}\log d}), 
    |w_{2j}| = O(\frac{1}{\sqrt{dk}\log d}), 
    \|w_{3:d, j}\| = O(\frac{1}{\sqrt{k}\log d})
\end{align*}
with probability greater than 1 - $\frac{1}{poly(d)}$.
\end{theorem}

\begin{theorem}
\label{th:lms_result:reg}
Under the conditions of Theorem~\ref{th:lms_result} and when minimizing regularization augmented loss term as shown below:
\begin{align*}
    L_f(S_m) = \frac{1}{m}\sum_i \max(0, 1-y_if(x^{(i)})) + \lambda \left (\frac{\partial f(x^{(i)})}{\partial x^{(i)}_1}\right)^2
\end{align*}
The learned weights satisfy:
\begin{align*}
    |w_{1j}| = \frac{2(1-\lambda)}{\sqrt k}(1-\frac{c}{\sqrt{\log d}}) + O(\frac{1}{\sqrt{dk}\log d})
\end{align*}
while $w_{2j}$ and $w_{3:d,j}$ take the same form as in Theorem~\ref{th:lms_result}
\end{theorem}

\begin{theorem}
\label{th:lms_result:perturb}
Under the conditions of Theorem~\ref{th:lms_result} and minimizing an objective that perturbs inputs along the first dimension below: 
\begin{align*}
    L_f(S_m) = \frac{1}{m}\sum_i \max(0, 1-y_if(x^{(i)}\odot b_i)), \quad \text{where }b_i\sim Bin([\alpha, 1, \dots, 1]), 1>\alpha>0
\end{align*}
The learned weights then satisfy:
\begin{align*}
&|w_{1j}| = \frac{2\alpha}{\sqrt k}(1-\frac{c}{\sqrt {\log d}}) + g(d, k),
  |w_{2j}|=\frac{2(1-\alpha)}{\sqrt{2\pi dk}}(1-\frac{c}{\sqrt{\log d}}) + g(d, k), \|w_{3:d, j}\| = O(\frac{1}{\sqrt{k}\log d})\\
& g(d, k)\leq \frac{\alpha}{\sqrt{dk}\log d}
\end{align*}    
We assume $1-\alpha=\Omega(\frac{1}{\sqrt{\log d}})$ is sufficiently small for the ease of analysis.

\end{theorem}

{\bf Remarks}.
Although the theorems above only analyse under somewhat mild regularization or perturbations, they help us understand the effect of different approaches on the weights.

1. Both regularization and perturbation diminish the weights of the first component
2. However, perturbation method also improve the weight of the second component.

Robustness methods are not without their share of drawbacks. When the space of irrelevant features is high-dimensional, perturbation methods may not cover the exponentially large volume of irrelevant region thereby failing to fully suppress irrelevant features. \JH{This is very good point and it explains why CoRM which perturb large volume of irrelevant region randomly does not work effectively (Table3). However, can this also explain IBP as well? Unlike the normal perturbations, IBP covers large volume of irrelevant features space. Then IBP can suppress irrelevant features when the large regulation hyperparameter(lambda) is given. However, it also overly regulates model parameters so that it hurts performance a lot. So how about adding this sentence like "Here, PGD can be applied to effectively find the useful perturbation on this high-dimensional space. Likewise, IBP which guarantees to cover large volume of irrelevant region can be helpful for this drawbacks. However, they can overly restrict model flexibility and training process unstable(cite other robustness papers saying tradeoff between robustness and general accuracy) "} Since regularization methods explicitly diminish irrelevant features, we found it more advantageous to combine perturbation methods with a regularization method especially when the irrelevant feature space is high-dimensional.

We further corroborate our findings in this section with empirical results on Decoy-MNIST dataset in the Experiments section. 

